Meta-material Sensors based Internet of Things for 6G Communications

In the coming 6G communications, the internet of things (IoT) serves as a key enabler to collect environmental information and is expected to achieve ubiquitous deployment. However, it is challenging for traditional IoT sensors to meet this expectation because of their requirements of power supplies and frequent maintenance, which are due to their power-demanding sense and transmit modules. To address this challenge, we propose a meta-IoT sensing system, where the IoT sensors are based on specially designed meta-materials. The meta-IoT sensors achieve simultaneous sensing and transmission by physical reflection and require no power supplies. In order to design a meta-IoT sensing system with optimal sensing accuracy, we jointly consider the sensing and transmission of meta-IoT sensors and propose efficient algorithms to optimize the meta-IoT structure and the sensing function at the receiver. As an example, we apply the meta-IoT system to sensing environmental temperature and humidity levels. Simulation results show that by using the proposed algorithm, the sensing accuracy can be largely increased.

==> sections/protocol.tex <==
%=======================
\section{Sensing Protocol for Meta-IoTs}
%=======================
\label{ssec: sensing procedure}

In this section, we propose the sensing protocol to incorporate {\mmr}s in wireless sensing systems and coordinate the {\ist}.
The sensing protocol consists of three phases, i.e., the \emph{data collecting phase}, the \emph{training phase}, and the \emph{measuring phase}, which are illustrated in Fig.~\ref{fig: protocol illustration} and described as follows.

\begin{figure}[!t]
\center{\includegraphics[width=0.8\linewidth]{./figures/sensing_protocol/sensing_protocol.pdf}}
	\vspace{-1.5em}
	\caption{Illustration of the sensing protocol for meta-IoTs.}
	\vspace{-1.em}
	\label{fig: protocol illustration}
\end{figure}

In the data collecting phase, we measure the environmental conditions and the corresponding received signal power as label and data, respectively, which constitutes the \emph{training data set} for the {\sensfunc}.
% 稍微详细一点说我们怎么做的.
Specifically, the set of measured environmental conditions is denoted by $\mathcal C$, which contains $N_C=|\mathcal C|$ different temperature-humidity pairs.
The set of Tx signal frequencies is denoted by $\mathcal F$, which is composed of $N_F = |\mathcal F|$ equally-spaced frequencies within $[f_{ub}, f_{lb}]$.
Then, for each environmental condition vector $\bm c\in \mathcal C$, we measure the power of received signals in dB at the $N_F$ frequencies for $N_M$ times, where the $m$-th measurement result is denoted by 
\begin{equation}
\label{equ: p_j,m}
	\bm p_{j,m} = \left(P_{\rx, dB}^{(m)}(f_1, \bm d; \bm c_j), ..., P_{\rx, dB}^{(m)}(f_{N_F}, \bm d; \bm c_j)\right),
\end{equation}
where the superscript $(m)$ indicates the $m$-th measurement.
%and referred to as the \emph{received power vector} for $(t_j,h_j)$.
%% 每一个温度湿度的数据被收集了 N_M 次, 共同组成了训练数据集.
%Moreover, the measurement of the received power vector given the $j$-th climate value is repeated for $N_M$ times, and the $m$-th received power vector is denoted by $\bm p_{j, m}$.
In summary, we denote the labeled data set collected in the training phase as 
\begin{equation}
\label{equ: train data set}
	\mathcal D_{train}= \{(\bm p_{j,m},\bm c_j)\}_{j\in[1,N_C], m\in[1,N_M]}.
\end{equation}

In the training phase, the {\rxunit} uses $\mathcal D_{train}$ to train the {\sensfunc}.
Without loss of generality, we consider the {\sensfunc} as a parameterized function with a parameter vector $\bm w$, which is denoted by $\bm g^{\bm w}$.
The {\sensfunc} maps a received power vector $\bm p$ to a $N_T$ dimensional sensing target condition vector, i.e., $\bm g^{\bm w}: \bm p \rightarrow \bm c$.
The parameter vector of the {\sensfunc}, i.e., $\bm w$, is optimized in order to minimize the loss between the sensing result and the label in $\mathcal D_{train}$.
The detailed training method will be discussed in Section~\ref{ssub: alg for sensing func opt}.

% 这个就是形成training的问题以及过程.
In the measuring phase, the {\systemname} continuously senses the climate condition.
Specifically, the system measures the received power vector $\bm p$ periodically, and the {\rxunit} uses the trained {\sensfunc} $\bm g^{\bm w}$ to estimate the current conditions of the $N_T$ sensing targets.
% 在此周期性的测量 received power vector, 并使用训练好的 {\sensfunc} 来估计当前的温度和湿度.

\endinput
